Mean distance in polyhedra

Given any polyhedron from which we select two random points uniformly and independently, we show that all the moments of the distance between those points can be always written in terms of elementary functions. As an illustration, the mean distance is found in the exact form for all Platonic solids.

==> polygons.tex <==
\section{Mean distance in regular polygons}
\subsection{Reduction}
As a demonstration, we show how CRT can be used to obtain the mean distance in regular polygons, that is, when $d=2$. Let $K$ be a regular $n$-sided polygon ($n\geq 3$) with vertices $V_i = [\cos\frac{2\pi i}{n},\sin\frac{2\pi k}{n}]$, where $i=0,1,2,\ldots,n-1$, so the polygon is circumscribed by a circle with radius one. For edges, we write $E_i = \overline{V_iV_{i+1}}$ with convention $V_{n}=V_0$. Note that for the area, we have $\volK = \frac{n}{2}\sin{\frac{2\pi}{n}}$ and for edge length $l=\volnon E_i=2\sin\frac{\pi}{n}$. Let $P=L^p$, then $P$ is even and homogenous of order $p$. In order to express $P_{22}$, we again use the Crofton Reduction technique. First, we select $C = [0,0]$ as our first scaling point. That way, $pP_{22} = 4(P_{21}-P_{22})$, where $P_{21}$ is a configuration with $A=K$ and $B$ is an (arbitrary) edge of $K$, we thus choose $B=E_0$. Our next scaling point is $C=V_0=[1,0]$, we have $pP_{21}=2(P_{11}-P_{21})+(P_{20}-P_{11})$. So far,
\begin{equation}
    P_{22} = \frac{4(2P_{11}+P_{20})}{(4+p)(3+p)},
\end{equation}
where $P_{20}=P_{KV_0}$ and
\begin{equation}
\label{eq:P11}
    P_{11} = \frac{2}{n}\sec\left(\frac{\pi}{n}\right)\sum_{i=1}^{n-2}  \sin\left(\frac{\pi i}{n}\right) \sin\left(\frac{\pi (i+1)}{n}\right) P_{E_i E_0}.
\end{equation}
The last relation follows from CRT and Definition \ref{def:weights} with $h_C(\partial_iK) = 2 \sin\frac{\pi i}{n} \sin\frac{\pi (i+1)}{n}$, where $\partial_iK=E_i$ with outer normal orientation. To reduce $P_{20}$, we choose $C=V_0$ and get $pP_{20}=2(P_{10}-P_{20})$, where (the weights are the same)
\begin{equation}
    P_{10} = \frac{2}{n}\sec\left(\frac{\pi}{n}\right)\sum_{i=1}^{n-2} \sin\left(\frac{\pi i}{n}\right) \sin\left(\frac{\pi (i+1)}{n}\right) P_{E_i V_0}.
\end{equation}
Finally, we can also reduce $P_{E_i E_0}$ into linear combination of $P_{E_i E_0}$. However, the reduction is dependent on whether $n$ is even or odd. Formally, let us write $p P_{E_i E_0} = 2(P_{E_i \partial E_0}-P_{E_i E_0})$ regardless of parity of $n$, so overall
\begin{equation}
\label{eq:P22PdP}
    P_{22} = \frac{16 \sec\left(\pi/n\right)}{n(4+p)(3+p)(2+p)} \sum_{i=1}^{n-2} \sin\left(\frac{\pi i}{n}\right) \sin\left(\frac{\pi(i+1)}{n}\right) (2P_{E_i \partial E_0}+P_{E_i V_0}).
\end{equation}

\subsection{Irreducible terms}
First, we shall compute the irreducible terms $P_{E_i V_0}$. These terms can be written as an integral over all points $X$ selected uniformly from $E_i$. A natural parametrisation is of course $X = V_i+s(V_{i+1}-V_{i})$, $s \in (0,l)$. Thus
\begin{equation}
P_{E_i V_0} = \frac{1}{l}\int_{0}^{l} \|V_i+s(V_{i+1}-V_{i})-V_0\|^p  \ddd s.
\end{equation}
However, we may parametrise $X$ in polar coordinates centered in $V_0$ instead. Let us write $r(\varphi) = \|X - V_0\|$ for $X \in E_i$, given that $X - V_0$ points in the direction of the polar angle $\varphi$. Note that the polar angle of vertex $V_i$ is $\varphi_i = \frac{\pi}{2} + \frac{\pi i}{n}$. Straightforward calculation reveals that
\begin{equation}
r(\varphi) = 2 \sin \left(\frac{\pi  i}{n}\right) \sin \left(\frac{\pi  (i+1)}{n}\right) \sec\left(\frac{2 \pi  i-n \varphi +\pi }{n}\right)
\end{equation}
and
\begin{equation}
\dd s = \sqrt{r(\varphi)^2 + \left(\frac{\dd r}{\dd \varphi}\right)^2} \ddd \varphi = 2 \sin \left(\frac{\pi  i}{n}\right) \sin \left(\frac{\pi  (i+1)}{n}\right) \sec^2\left(\frac{2 \pi  i-n \varphi +\pi }{n}\right) \ddd \varphi.
\end{equation}
Therefore,
\begin{equation}
P_{E_i V_0} = 2^p\sin^{1+p}\left(\frac{\pi i}{n}\right)\sin^{1+p}\left(\frac{\pi (i+1)}{n}\right)\csc\left(\frac{\pi}{n}\right)\int_{\varphi_i}^{\varphi_{i+1}}  \sec^{2+p}\left(\frac{2 \pi  i-n \varphi +\pi }{n}\right)\ddd \varphi.
\end{equation}
\begin{comment}
where $\uvect{n}_\varphi$ is a normal vector pointing in the direction of a radial line whose points have polar angle $\varphi$. When $P = L^p$, then $\tilde{P}(\uvect{n}_\varphi) = 1$.
\end{comment}
Using reparametrisation $(2 \pi  i-n \varphi +\pi )/n=\zeta$, we get
\begin{equation}
\label{eq:PEiV0}
P_{E_i V_0} = 2^p\sin^{1+p}\left(\frac{\pi i}{n}\right)\sin^{1+p}\left(\frac{\pi (i+1)}{n}\right)\csc\left(\frac{\pi}{n}\right)\int_{\pi i/n}^{\pi(i+1)/n}  \csc^{2+p}\zeta\ddd \zeta.
\end{equation}
By definition, we put $P_{E_0 V_0} = P_{E_n V_0} = 0$.

\subsection{Odd number of sides}
If $n$ is odd, we select for all $i$ the following scaling point
\begin{equation}
C_i = \mathcal{A}(E_i)\cap \mathcal{A}(E_0) = \cos \left(\frac{\pi }{n}\right) \sec \left(\frac{\pi i }{n}\right) \left[\cos
   \left(\frac{\pi (i+1)}{n}\right),\sin \left(\frac{\pi (i+1)}{n}\right)\right]
\end{equation}
from which
\begin{equation}
    P_{E_i \partial E_0} = \frac{1}{2} \csc \left(\frac{\pi }{n}\right) \sec\left(\frac{\pi i }{n}\right)\left( 
   \sin \left(\frac{\pi (i+1)}{n}\right) P_{E_i V_0} -
   \sin \left(\frac{\pi (i-1)}{n}\right) P_{E_i V_1}\right).
\end{equation}
We can simplify Equation \eqref{eq:P22PdP} in the following way: Note that, rotating $K$ by $2\pi/n$, we see that $P_{E_i V_1} = P_{E_{i-1} V_0}$, using which we can deduce, after splitting and then by shifting the summation from $i$ to $i+1$,
\begin{equation}
\label{eq:P22}
    P_{22} = \frac{-16 \sec\left(\pi/n\right)}{n(4+p)(3+p)(2+p)} \sum_{i=1}^{n-2} \frac{\sin^2\left(\pi i/n\right) \sin^2\left(\pi(i+1)/n\right)}{\cos\left(\pi i/n\right) \cos\left(\pi(i+1)/n\right)} P_{E_i V_0},
\end{equation}
\begin{comment}
Alternatively, we can express $P_{22}$ as a sum over $P_{E_i \partial E_0}$ instead of $P_{E_i V_0}$,
\end{comment}
from which immediately in total, for odd $n$ and $p>-2$ arbitrary,
\begin{equation}
\label{eq:L22}
    P_{22} = \frac{-2^{4+p} \sec\left(\pi/n\right)\csc\left(\pi/n\right)}{n(4+p)(3+p)(2+p)} \sum_{i=1}^{n-2} \frac{\sin^{3+p}\left(\pi i/n\right) \sin^{3+p}\left(\pi(i+1)/n\right)}{\cos\left(\pi i/n\right) \cos\left(\pi(i+1)/n\right)} \int_{\pi i/n}^{\pi(i+1)/n}  \csc^{2+p}\zeta\ddd \zeta.
\end{equation}

\subsection{Even number of sides}
If $n$ is even, then $P_{E_{n/2} E_0}$ is irreducible since $E_0$ and $E_{n/2}$ are parallel. However, we can use overlap formula to deduce that
\begin{equation}
    P_{E_{n/2} E_0} = \frac{1}{l^2} \int_{-l}^l
    (h^2+x^2)^{p/2} |l-x| \ddd x,
\end{equation}
where $h=2\cos(\pi/n)$ is the separation between $E_{n/2}$ and $E_0$. Identifying $\frac{1}{l} \int_0^l (h^2+x^2)^{p/2} \ddd x$ as $P_{E_{n/2}V_0}$ and solving the remaining integral, we get
\begin{equation}
    P_{E_{n/2} E_0} = 2P_{E_{n/2}V_0}-\frac{2^{p+1} \csc ^2\left(\frac{\pi }{n}\right)}{2+p}\left(1-\cos ^{2+p}\left(\frac{\pi }{n}\right)\right),
\end{equation}
The Equation \eqref{eq:P22PdP} is still valid provided we treat $P_{E_{n/2} \partial E_0}$ only formally as the solution of the equation $p P_{E_{n/2} E_0} = 2(P_{E_{n/2} \partial E_0}-P_{E_{n/2} E_0})$. That is,
\begin{equation}
P_{E_{n/2}\partial E_0} = \frac{2+p}{2} P_{E_{n/2} E_0} = (2+p)L_{E_{n/2}V_0}-2^p \csc ^2\left(\frac{\pi }{n}\right) \left(1-\cos ^{2+p}\left(\frac{\pi }{n}\right)\right).
\end{equation}
Exploiting symmetries $P_{E_i V_0} = P_{E_{n-i-1} V_0}$ and $P_{E_i \partial E_0} = P_{E_{n-i}\partial E_0}$ and and shifting $i \to i+1$, we get from Equation \eqref{eq:P22PdP} for any even $n$ and $p>-2$,
\begin{equation}
\label{eq:P22even}
\begin{split}
& P_{22} = \frac{32 \sec \left(\frac{\pi }{n}\right)}{n
   (4+p) (3+p) (2+p)} \bigg{(}\cos \left(\frac{\pi }{n}\right) \left(3+p+\cot ^2\left(\frac{\pi
   }{n}\right)\right) P_{E_{n/2}V_0} \\
   &-2^p \frac{\cos(\pi/n)}{\sin^2(\pi/n)} \left(1-\cos^{2+p}\left(\frac{\pi }{n}\right)\right) -\sum _{i=1}^{\frac{n}{2}-2} \frac{\sin^2\left(\pi i/n\right) \sin^2\left(\pi(i+1)/n\right)}{\cos\left(\pi i/n\right) \cos\left(\pi(i+1)/n\right)} P_{E_i V_0}\bigg{)}.
\end{split}
\end{equation}

\subsection{Arbitrary number of sides}
Alternatively, if we redefine $P_{E_i \partial E_0}$ to be equal to $\lim_{x \to i} P_{E_x \partial E_0}$, where
\begin{equation}
\label{eq:PExdE0}
    P_{E_x \partial E_0} = \frac{1}{2} \csc \left(\frac{\pi }{n}\right) \sec\left(\frac{\pi x }{n}\right)\left( 
   \sin \left(\frac{\pi (x+1)}{n}\right) P_{E_x V_0} -
   \sin \left(\frac{\pi (x-1)}{n}\right) P_{E_x V_1}\right).
\end{equation}
and
\begin{equation}
\label{eq:PExV0}
P_{E_x V_0} = 2^p\sin^{1+p}\left(\frac{\pi x}{n}\right)\sin^{1+p}\left(\frac{\pi (x+1)}{n}\right)\csc\left(\frac{\pi}{n}\right)\int_{\pi x/n}^{\pi(x+1)/n}  \csc^{2+p}\zeta\ddd \zeta
\end{equation}
for $x \in \mathbb{R}$. One can show, by taking the limit, that we get the same expression for $P_{E_{n/2}V_0}$ when $n$ is even. Thus, using this redefinition of $P_{E_i \partial E_0}$, Equation \eqref{eq:P22PdP} is valid for $n \geq 3$ regardless of $n$ being even or odd. 

\subsection{Even moments}
Let us briefly discuss the case of even moments. Uwe B\"{a}sel \cite{basel2021moments} found the values of $L_{22}^{(p)}$ for $p=2$ and $p=4$, namely
\begin{equation}
L^{(2)}_{22} = \frac{1}{3}\left(2+\cos\frac{2\pi}{n}\right), \qquad L^{(4)}_{22} = \frac{1}{90} \left(77+64 \cos\frac{2 \pi }{n}+9 \cos\frac{4 \pi }{n}\right).
\end{equation}
Using Equation \eqref{eq:P22PdP} with redefinition $P_{E_i \partial E_0} = \lim_{x \to i} P_{E_x \partial E_0}$, we can rederive those formulae easily. For example, when $p = 2$, we get from Equation $\eqref{eq:PExV0}$,
\begin{equation}
L^{(2)}_{E_x V_0} = \frac{5}{3}+\frac{1}{3} \cos\frac{2 \pi }{n}-\cos\frac{2 \pi  x}{n}-\cos \frac{2 \pi(x+1)}{n}
\end{equation}
and from Equation $\eqref{eq:PExdE0}$, after simplifications,
\begin{equation}
L^{(2)}_{E_x \partial E_0} = \frac{8}{3}+\frac{4}{3} \cos\frac{2 \pi }{n}-\cos\frac{2\pi(i-1)}{n}-2 \cos\frac{2 \pi i}{n}-\cos\frac{2 \pi (i+1)}{n}.
\end{equation}
Therefore, plugging those into Equation \eqref{eq:P22PdP},
\begin{equation}
\begin{split}
    L^{(2)}_{22} & = \frac{16 \sec\left(\pi/n\right)}{n(4+p)(3+p)(2+p)} \sum_{i=1}^{n-2} \sin\left(\frac{\pi i}{n}\right) \sin\left(\frac{\pi(i+1)}{n}\right) \bigg{(}7+3 \cos \frac{2 \pi }{n}\\
    & -2 \cos\frac{2\pi (i-1)}{n}-5 \cos\frac{2 \pi i}{n}-3 \cos\frac{2\pi (i+1)}{n}\bigg{)}.
\end{split}
\end{equation}
Finally, we can sum this series using CAS software (\textit{Mathematica} of \textit{Maple}). As a result, we were able to deduce the following simple formulae for higher even moments (the formulae are valid for $n\geq 3$ regardless of $n$ being odd or even),
\begin{align}
L^{(6)}_{22} & = \frac{1}{420} \left(628+661\cos\frac{2 \pi }{n} +164 \cos\frac{4 \pi}{n} +17 \cos\frac{6 \pi}{n}\right) -\frac{\delta_{n3}}{50}\\
\begin{split}
L^{(8)}_{22} & = \frac{1}{1575}\bigg{(}4921+5936 \cos\frac{2 \pi }{n}+1974 \cos\frac{4 \pi }{n} +368 \cos\frac{6 \pi }{n}+31 \cos\frac{8 \pi}{n}\bigg{)}-\frac{16 \delta _{3n}}{175}+\frac{2 \delta_{4n}}{225}
\end{split}\\
\begin{split}
L^{(10)}_{22} & = \frac{1}{4158}\bigg{(}30476+40162 \cos\frac{2 \pi }{n}+16072 \cos\frac{4 \pi }{n}+4093 \cos\frac{6 \pi }{n}\\
&\hspace{4em}+628\cos\frac{8 \pi }{n}+45 \cos\frac{10 \pi }{n}\bigg{)}-\frac{15 \delta_{3n}}{49}+\frac{4 \delta_{4n}}{63}-\frac{2 \delta_{5n}}{441}
\end{split}\\
\begin{split}
L^{(12)}_{22} & = \frac{1}{840840}\bigg{(}15673314+21975552 \cos\frac{2 \pi }{n}+10006023 \cos\frac{4 \pi }{n}+3122432 \cos\frac{6 \pi}{n}\\
& \hspace{-2em} +661402 \cos\frac{8 \pi }{n}+87296 \cos\frac{10 \pi }{n}+5461 \cos\frac{12 \pi}{n}\bigg{)}\!-\frac{2847 \delta_{3n}}{3080}\!+\!\frac{668 \delta_{4n}}{2205}-\frac{17\!+\!\sqrt{5}}{441} \delta_{5n}\!+\!\frac{\delta_{6n}}{392},
\end{split}\\
\begin{split}
L^{(14)}_{22} & = \frac{1}{308880}\bigg{(}15540360+22811745 \cos\frac{2 \pi }{n}+11429660 \cos\frac{4 \pi }{n}+4126221 \cos\frac{6 \pi}{n}\\
& +1081192 \cos\frac{8 \pi }{n}+198713 \cos\frac{10 \pi }{n}+23124 \cos\frac{12 \pi}{n}+1285 \cos\frac{14 \pi }{n}\bigg{)}\\
& -\frac{384 \delta _{3n}}{143}+\frac{1816 \delta_{4n}}{1485}-\frac{3057+331 \sqrt{5}}{14256}\delta_{5n}+\frac{11 \delta _{6n}}{360}-\frac{\delta _{7n}}{648},
\end{split}
\end{align}
where $\delta_{jk}$ is the Kronecker delta. Based on the obtained results, we state the following conjecture:

\begin{conjecture}
Let $K$ be a regular $n$-sided polygon ($n\geq 3$) circumscribed by a circle with unit radius. Then for $p$ being a positive even integer,
\begin{equation}
    L_{22}^{(p)} = \sum_{j=0}^{p/2} \left(a_{jp}\cos\left(\frac{2\pi j}{n}\right) + b_{jp}\delta_{jn}\right)
\end{equation}
for some numbers $a_{jp}$ and $b_{jp}$.
\end{conjecture}
\begin{remark}
Note that, since $n \geq 3$, the values of $b_{0p}$, $b_{1p}$ and $b_{2p}$ can be arbitrary.
\end{remark}

\noindent
Using Equation \eqref{eq:P22PdP}, we also found the following limit
\begin{equation}
    \lim_{p \to -2^+} (2+p)L^{(p)}_{22} = \frac{4 \pi}{n \sin \frac{2 \pi }{n}},
\end{equation}
which is in agreement with general statement valid for any compact convex $K$, that
\begin{equation}
    \lim_{p \to -2^+} (2+p)L^{(p)}_{22} = \frac{8\pi}{\volK},
\end{equation}
see XXX for a refference.

\subsection{Odd moments}
When $p=-1$, we got
\begin{equation}
    L^{(-1)}_{E_i V_0} = \frac{\csc (\pi/n)}{2}\ln \frac{\tan (\pi (i+1)/n)}{\tan (\pi i /n)},
\end{equation}
from which, immediately when $n$ is odd,
\begin{equation}
    L^{(-1)}_{22} = \frac{-4 \sec\left(\pi/n\right) \csc (\pi/n)}{3n} \sum_{i=1}^{n-2} \frac{\sin^2\left(\pi i/n\right) \sin^2\left(\pi(i+1)/n\right)}{\cos\left(\pi i/n\right) \cos\left(\pi(i+1)/n\right)} \ln \frac{\tan (\pi (i+1)/n)}{\tan (\pi i /n)}.
\end{equation}

\subsection{Limiting behaviour for large number of sides}
In order to extract the limiting properties of $P_{22}$, we let $n$ go to infinity but at the same time hold $\sigma_i = i/n$ as fixed. We denote $\varepsilon = 1/n$. By Taylor Expansion of Equation \eqref{eq:PEiV0},
\begin{equation}
    P_{E_i V_0} \! =\! 2^p\left(1+\frac{p \pi  \varepsilon  \cot (\pi  \sigma_i )}{2}-\frac{p \pi ^2 \varepsilon^2}{12} (3-p-(1+p) \cos (2 \pi  \sigma_i )) \csc ^2(\pi  \sigma_i
   )\right) \sin^p(\pi  \sigma_i ) + O(\varepsilon^3),
\end{equation}
from which
\begin{equation}
    P_{E_i \partial E_0} = 2^{p-1} (2+p) \left(1-\frac{p \pi ^2 \varepsilon^2}{24} (6-p-(4+p) \cos (2 \pi  \sigma_i )) \csc^2(\pi  \sigma_i )\right) \sin^p(\pi  \sigma_i ) + O(\varepsilon^3).
\end{equation}
All together, by Equation \eqref{eq:P22PdP},
\begin{equation}
\label{eq:P22spec}
\begin{split}
    P_{22} & = \frac{2^{4+p} \varepsilon}{(4+p)(3+p)(2+p)} \sum_{i=1}^{n-2}\bigg{(} (3+p) \sin ^{2+p}(\pi  \sigma_i )+\frac{3\pi \varepsilon}{4} (2+p)  \sin ^p(\pi  \sigma_i ) \sin (2 \pi  \sigma_i ) \\
    & +\frac{p \pi ^2 \varepsilon^2}{24} \left(-12-2p+p^2+(4+p)^2 \cos (2 \pi  \sigma_i )\right) \sin ^p(\pi  \sigma_i ) + O(\varepsilon^3)\bigg{)}.    
\end{split}
\end{equation}
Let $f(x)$ be any sufficiently smooth function. Note that
\begin{equation}
\int_0^1 f(x) \ddd x = \sum_{i=0}^{n-1} \int_{\sigma_i}^{\sigma_i+\varepsilon} f(x) \ddd x,
\end{equation}
so by expanding $f(x)$ into Taylor series around $x = \sigma_i = i/n$ and integrating, we get
\begin{equation}
    \int_0^1 f(x) \ddd x = \varepsilon\sum_{i=0}^{n-1} \left(f(\sigma_i) + \frac{\varepsilon}{2}f'(\sigma_i) + \frac{\varepsilon^2}{6}f''(\sigma_i) + \frac{\varepsilon^3}{24}f'''(\sigma_i)+\frac{\varepsilon^4}{120}f^{(4)}(\sigma_i) + O(\varepsilon^5) \right).
\end{equation}
Replacing $f$ with $f'$, $f''$ and so on, we can, by linear combination, invert this relation to
\begin{equation}
    \varepsilon\sum_{i=0}^{n-1} f(\sigma_i) = \int_0^1 f(x) - \frac{\varepsilon}{2} f'(x) + \frac{\varepsilon^2}{12} f''(x) - \frac{\varepsilon^4}{720} f^{(4)}(x) + O(\varepsilon^5) \ddd x,
\end{equation}
which is not surprising since it is essentially the Euler-Maclaurin formula. Since our sums run from $1$ to $n-2$, so by subtracting terms with $i=0$ and $i=n-1$ to the right hand side and performing necessary Taylor expansions, we get
\begin{equation}
\begin{split}
    \varepsilon\sum_{i=1}^{n-2} f(\sigma_i) & = \int_0^1 f(x)\ddd x - \frac{\varepsilon}{2} (f(0)+3 f(1)) -\frac{\varepsilon^2}{12} \left(f'(0)-13 f'(1)\right)\\
    & -\frac{\varepsilon^3}{2} f''(1)+\frac{\varepsilon^4}{720}
   \left(f^{(3)}(0)+119 f^{(3)}(1)\right) + O(\varepsilon^5).
\end{split}
\end{equation}
Therefore, summing Equation \eqref{eq:P22spec} using this relation, we get the following formula
\begin{equation}
P_{22} = \left(1 - \frac{p \pi^2}{3n^2} + O\left(\frac{1}{n^4}\right)\right)P_{22d},
\end{equation}
where
\begin{equation}
P_{22d} = L^{(p)}_{22d} = \frac{2^{4+p} \Gamma\left(\frac{3+p}{2}\right)}{(2+p)(4+p)\sqrt{\pi}\, \Gamma\left(2+\frac{p}{2}\right)}
\end{equation}
is the mean distance $p$-th moment in a unit disk. This approximation is valid for all $p>-2$. Using the same technique, we were able to further improve the estimate to
\begin{equation}
P_{22} = \left(1 - \frac{p \pi^2}{3n^2} + \frac{p^2 (8+11 p) \pi ^4}{180 (1+p) n^4}+\frac{p \left(16+p \left(8+p-15 p^2\right)\right) \pi ^6}{1890 (1+p) n^6} + O\left(\frac{1}{n^8}\right)\right)P_{22d}
\end{equation}
with the property that the expansion is valid for $p>k-5$ if it is truncated at $1/n^{k}$ term. The reason why the approximation is not correct there is because $f$ is not sufficiently smooth at the endpoints for low $p$. However, we can treat those cases separately. Most notably, when $p=-1$, we got the following expansion

XXX

Finally, for $p=1$, we got XXX
\begin{equation}
L^{(1)}_{22} = \left(1 - \frac{\pi^2}{3n^2} + \frac{19\pi^4}{360n^4}+? + O\left(\frac{1}{n^8}\right)\right)P_{22d}
\end{equation}

\begin{comment}
\vspace{5em}
\noindent
Note that, due to presence of singular $\tan(\pi i/n)$ term when $i=n/2$, we cannot express $P_{E_i \partial E_0}$ as a linear combination of $P_{E_i V_0}$ and $P_{E_i V_1}$ as shown in Equation XXX.

%One can check that in fact this relation is correct for any $n$ regardless of being even or odd.

Let us write $\csc^{2+p}\zeta = \csc^{3+p}\zeta \sin\zeta$. Using integration by parts, we get
\begin{equation}
    \int_{\pi i/n}^{\pi(i+1)/n}  \csc^{3+p}\zeta \sin\zeta\ddd \zeta = 
\end{equation}
\end{comment}

\begin{comment}
% Alternative computer assisted summation ["NEWONE" PROGRAM IN MATHEMATICA NOTEBOOK]:
We present a more detailed procedure how this is done -- the method is based on cancelling the cosines in the denominator. First, using symmetry $P_{E_i V_0} = P_{E_{n-i-1} V_0}$, we rewrite Equation \eqref{eq:P22} as
\begin{equation}
    P_{22} = \frac{16 \sec\left(\pi/n\right)}{n(4+p)(3+p)(2+p)} \sum_{i=1}^{n-2} \left( 1+2 \cot \left(\frac{\pi }{n}\right) \tan \left(\frac{\pi i }{n}\right)\right)\sin\frac{\pi i}{n} \sin \frac{\pi (i+1)}{n} \, P_{E_i V_0}.
\end{equation}
so now, there is only one cosine term in the denominator (in the tangens term). One can check, by adding a sum whose indices have been reflected $i \to n - i - 1$, that this is indeed the same expression. Note that when $n$ is odd, there is no singularity since $i = n/2$ is not an integer. To cancel the tangens term, however, we need to view the equation as if $i$ was real. That way, we can always cancel singularity at $i = n/2$ by subtracting an appropriate constant from $\sin\frac{\pi i}{n} \sin \frac{\pi (i+1)}{n} \, P_{E_i V_0}$. Substituting $i=n/2$, we get that this constant is $\cos(\pi/n) P_{E_{n/2} V_0}$. Even though the term $P_{E_{n/2} V_0}$ should not be defined for $i$ not being an integer, we can extend the definition of $P_{E_i V_0}$ to any real $i$ by means of Equation \eqref{eq:PEiV0}. That is,
\begin{equation}
   \cos\left(\frac{\pi}{n}\right) P_{E_{n/2} V_0} = 2^p \cos ^{2+p}\left(\frac{\pi }{n}\right) \csc \left(\frac{\pi }{n}\right) \int_{\frac{\pi }{2}}^{\frac{\pi }{2}+\frac{\pi }{n}} \csc^{2+p}\zeta \ddd \zeta.
\end{equation}
Writing
\begin{equation}
\sin\frac{\pi i}{n} \sin \frac{\pi (i+1)}{n} \, P_{E_i V_0} = \sin\frac{\pi i}{n} \sin \frac{\pi (i+1)}{n} \, P_{E_i V_0} - \cos\frac{\pi}{n} P_{E_{n/2} V_0} + \cos\frac{\pi}{n} P_{E_{n/2} V_0}
\end{equation}
and using the relation $\sum_{i=1}^{n-1} \tan \frac{\pi i}{n} = 0$ (valid for odd $n$), we get
\begin{equation}
\begin{split}
    P_{22} & = \frac{16 \sec\left(\pi/n\right)}{n(4+p)(3+p)(2+p)} \Bigg{(} n \cos\left(\frac{\pi}{n}\right) P_{E_{n/2}V_0}\\
    & +\sum_{i=1}^{n-2} \left( 1+2 \cot \left(\frac{\pi }{n}\right) \tan \left(\frac{\pi i }{n}\right)\right)\left(\sin\frac{\pi i}{n}\sin \frac{\pi (i+1)}{n} \, P_{E_i V_0} - \cos\frac{\pi}{n} P_{E_{n/2} V_0}\right)\Bigg{)}
\end{split}
\end{equation}
with $P_{E_i V_0}$ defined in Equation \eqref{eq:PEiV0}. In this form for any even $p$, there is always a cancellation of the cosine term in the denominator of tangens with $\sin\frac{\pi i}{n}\sin \frac{\pi (i+1)}{n} \, P_{E_i V_0} - \cos\frac{\pi}{n} P_{E_{n/2} V_0}$. Moreover, since now there is no singularity in $i$, the value of $P_{22}$ if finite also for $n$ being even. It can be shown, after proper cancellation, that this value of $P_{22}$ matches the correct one given by Equation \eqref{eq:P22even}.
\end{comment}
